ForceGrip: Reference-Free Curriculum Learning for Realistic Grip Force Control in VR Hand Manipulation

Realistic Hand manipulation is a key component of immersive virtual reality (VR), yet existing methods often rely on kinematic approach or motion-capture datasets that omit crucial physical attributes such as contact forces and finger torques. Consequently, these approaches prioritize tight, one-size-fits-all grips rather than reflecting users' intended force levels. We present ForceGrip, a deep learning agent that synthesizes realistic hand manipulation motions, faithfully reflecting the user's grip force intention. Instead of mimicking predefined motion datasets, ForceGrip uses generated training scenarios-randomizing object shapes, wrist movements, and trigger input flows-to challenge the agent with a broad spectrum of physical interactions. To effectively learn from these complex tasks, we employ a three-phase curriculum learning framework comprising Finger Positioning, Intention Adaptation, and Dynamic Stabilization. This progressive strategy ensures stable hand-object contact, adaptive force control based on user inputs, and robust handling under dynamic conditions. Additionally, a proximity reward function enhances natural finger motions and accelerates training convergence. Quantitative and qualitative evaluations reveal ForceGrip's superior force controllability and plausibility compared to state-of-the-art methods. Demo videos are available as supplementary material and the code is provided at https://han-dongheun.github.io/ForceGrip.

==> ACMprocess-metadata.tex <==
\title{ForceGrip: Reference-Free Curriculum Learning for Realistic Grip Force Control in VR Hand Manipulation}

\author{DongHeun Han}
\orcid{0000-0001-7693-7674}
\affiliation{\institution{IIIXR LAB, Kyung Hee University}
\city{Yongin}
\country{Republic of Korea}}
\email{hand32@khu.ac.kr}

\author{Byungmin Kim}
\orcid{0009-0001-7161-6588}
\affiliation{\institution{IIIXR LAB, Korea University}
\city{Seoul}
\country{Republic of Korea}}
\email{kbmstar1@korea.ac.kr}

\author{RoUn Lee}
\orcid{0000-0003-1596-5115}
\affiliation{\institution{IIIXR LAB, Kyung Hee University}
\city{Yongin}
\country{Republic of Korea}}
\email{dlfhdns@khu.ac.kr}

\author{KyeongMin Kim}
\orcid{0000-0001-5168-9563}
\affiliation{\institution{IIIXR LAB, Korea University}
\city{Seoul}
\country{Republic of Korea}}
\email{kgm031189@gmail.com}

\author{Hyoseok Hwang}
\orcid{0000-0003-3241-8455}
\affiliation{\institution{AIR Lab, Kyung Hee University}
\city{Yongin}
\country{Republic of Korea}}
\email{hyoseok@khu.ac.kr}

\author{HyeongYeop Kang}
\orcid{0000-0001-5292-4342}
\affiliation{\institution{IIIXR LAB, Korea University}
\city{Seoul}
\country{Republic of Korea}}
\email{siamiz_hkang@korea.ac.kr}
